EgoIntent: A Pre-Outcome Micro-Step Benchmark for Understanding What, Why, and Next

Egocentric video provides a natural modality for studying human behavior, but conventional visual understanding captures mainly observable scenes, objects, and actions rather than the latent goals that organize them. Existing intent benchmarks typically focus on coarse event-level goals and overlook how intent evolves across procedural steps. We introduce EgoIntent, a step-level intent-understanding benchmark comprising 3,014 pre-outcome micro-steps from 32 egocentric videos across 15 indoor and outdoor daily-life scenarios. Each step is manually annotated along three complementary dimensions: Local Intent (What), the immediate goal; Procedural Intent (Why), the role of the step in the broader procedure; and Next-Plan (Next), the action most likely to follow. Multiple rounds of human review refine temporal boundaries and annotation quality. We evaluate 15 multimodal large language models using reference-based scores and complementary reference-free diagnostics. Controlled studies on four representative models show that only one model gains significantly from correct temporal order, while a single boundary frame outperforms the full ordered clip for three models. Step-only input performs best for all four models, and adding 15 seconds of history significantly degrades three. Revealing the current outcome improves Local Intent by 7.81 points, while revealing the following step improves Next-Plan by 13.17 points. These findings indicate that current models can achieve strong intent-prediction scores through static boundary cues without robustly exploiting temporal order or procedural history.

==> sections/discussion.tex <==
\section{Discussion}
Our evaluation indicates that current MLLMs' step-level intent understanding on EgoIntent remains far from mature. Under pre-outcome truncation, models must infer intent before the decisive result becomes visible, exposing errors that would otherwise be hidden by outcome cues. Across models, \textit{global intent} is consistently easier than \textit{local intent} and \textit{next-step plan}, suggesting reliance on coarse procedural priors rather than temporally grounded goal inference and action-transition prediction—especially for short, preparatory, or transitional steps where evidence lies in subtle hand--object interactions and intermediate state changes. Moreover, the pronounced scenario-level variance implies limited robustness and transfer when cues are implicit, object states are ambiguous, or multiple plausible next actions exist. This also suggests that simply scaling parameters may not close the gap without stronger fine-grained temporal perception and progress tracking at step boundaries. Future work could further benefit from diagnostics that separate \emph{perception failures} from \emph{procedural reasoning failures}, and from explicitly modeling object-centric state/progress with uncertainty-aware goal-to-action transitions. More broadly, EgoIntent highlights the need for benchmarks that stress-test proactive intent inference under incomplete evidence, rather than retrospective recognition after outcomes are revealed.
